To BEE or not to BEE: Estimating more than Entropy with Biased Entropy Estimators

Entropy estimation plays a significant role in biology, economics, physics, communication engineering and other disciplines. It is increasingly used in software engineering, e.g. in software confidentiality, software testing, predictive analysis, machine learning, and software improvement. However accurate estimation is demonstrably expensive in many contexts, including software. Statisticians have consequently developed biased estimators that aim to accurately estimate entropy on the basis of a sample. In this paper we apply 18 widely employed entropy estimators to Shannon measures useful to the software engineer: entropy, mutual information and conditional mutual information. Moreover, we investigate how the estimators are affected by two main influential factors: sample size and domain size. Our experiments range over a large set of randomly generated joint probability distributions and varying sample sizes, rather than choosing just one or two well known probability distributions as in previous investigations. Our most important result is identifying that the Chao-Shen and Chao-Wang-Jost estimators stand out for consistently converging more quickly to the ground truth, regardless of domain size and regardless of the measure used. They also tend to outperform the others in terms of accuracy as sample sizes increase. This discovery enables a significant reduction in data collection effort without compromising performance.

==> sections/Fp_table_side.tex <==
\newcolumntype{N}{>{\mdseries}^w{c}{2mm}}
\begin{table*}[t!]
\small
\begin{tabular}{c c c}
    \begin{subtable}{0.315\textwidth}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{ |l *{6}{N} : l *{2}{N}}
        \hline
        \rowstyle{} \diagbox{\emph{est}}{\emph{k}} & \rotatebox{90}{256} & \rotatebox{90}{1024} & \rotatebox{90}{4096} & \rotatebox{90}{16384} & \rotatebox{90}{65536} & \rotatebox{90}{262K} & \rotatebox{90}{Slope} & \rotatebox{90}{$l_2$-norm} \\
        \hline
        ML & \cellcolor{gray!25}9 & \cellcolor{gray!25}10 & \cellcolor{gray!25}12 & & & & 1.5 & 31.6 \\
        MM & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}11 & \cellcolor{ao(english)!35}13 & & & 1.33 & 30.0 \\
        GS\small{88} & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}11 & \cellcolor{ao(english)!35}13 & & & 1.33 & 30.0 \\
        GS\small{03} & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}11 & \cellcolor{ao(english)!35}13 & & & 1.33 & 30.0 \\
        SHU & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}11 & \cellcolor{ao(english)!35}13 & & & 1.33 & 30.0 \\
        \textbf{CS} & \cellcolor{bluebell!60}\textbf{9} & \cellcolor{bluebell!60}\textbf{9} & \cellcolor{bluebell!60}\textbf{10} & \cellcolor{bluebell!60}\textbf{9} & \cellcolor{bluebell!60}\textbf{10} & \cellcolor{bluebell!60}\textbf{12} & \textbf{0.5} & \textbf{24.23} \\
        Z & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}11 & \cellcolor{ao(english)!35}13 & & & 1.33 & 30.0 \\
        SH & \cellcolor{gray!25}9 & \cellcolor{gray!25}10 & \cellcolor{gray!25}12 & & & & 1.5 & 31.6 \\
        B & 11 & 13 & & & & & & \\
        \textbf{CW} & \cellcolor{bluebell!90}\textbf{9} & \cellcolor{bluebell!90}\textbf{9} & \cellcolor{bluebell!90}\textbf{10} & \cellcolor{bluebell!90}\textbf{9} & \cellcolor{bluebell!90}\textbf{10} & \cellcolor{bluebell!90}\textbf{12} & \textbf{0.5} & \textbf{24.23} \\
        PYM & & & & & & & & \\
        BAY & \cellcolor{gray!25}9 & \cellcolor{gray!25}10 & \cellcolor{gray!25}12 & & & & 1.5 & 31.6 \\
        LAP & \cellcolor{gray!25}9 & \cellcolor{gray!25}10 & \cellcolor{gray!25}12 & & & & 1.5 & 31.6 \\
        J & \cellcolor{gray!25}9 & \cellcolor{gray!25}10 & \cellcolor{gray!25}12 & & & & 1.5 & 31.6 \\
        SG & \cellcolor{gray!25}10 & \cellcolor{gray!25}10 & \cellcolor{gray!25}12 & & & & 1.5 & 31.6 \\
        MIN & & & & 11 & 12 & 12 & & \\
        NSB & & & & & & & & \\
        ANSB & & & & & & & & \\
        \hline
    \end{tabular}
    \end{adjustbox}
    \caption{H}
    \label{tab:Fp_tab_h}
    \end{subtable} &
    \begin{subtable}{0.315\textwidth}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{ |l *{6}{N} : l *{2}{N} }
        \hline
        \rowstyle{} \diagbox{\emph{est}}{\emph{k}} & \rotatebox{90}{256} & \rotatebox{90}{1024} & \rotatebox{90}{4096} & \rotatebox{90}{16384} & \rotatebox{90}{65536} & \rotatebox{90}{262K} & \rotatebox{90}{Slope} & \rotatebox{90}{$l_2$-norm} \\
        \hline
        ML & \cellcolor{gray!25}8 & \cellcolor{gray!25}11 & \cellcolor{gray!25}13 & & & & 2.5 & 32.1 \\
        MM & \cellcolor{gray!45}8 & \cellcolor{gray!45}10 & \cellcolor{gray!45}12 & & & & 2.0 & 31.4 \\
        \textbf{GS\small{88}} & \cellcolor{ao(english)!35}\textbf{7} & \cellcolor{ao(english)!35}\textbf{9} & \cellcolor{ao(english)!35}\textbf{11} & \cellcolor{ao(english)!35}\textbf{13} & & & \textbf{2.0} & \textbf{29.5} \\
        GS\small{03} & \cellcolor{gray!45}8 & \cellcolor{gray!45}10 & \cellcolor{gray!45}12 & & & & 2.0 & 31.4 \\
        \textbf{SHU} & \cellcolor{ao(english)!35}\textbf{7} & \cellcolor{ao(english)!35}\textbf{9} & \cellcolor{ao(english)!35}\textbf{11} & \cellcolor{ao(english)!35}\textbf{13} & & & \textbf{2.0} & \textbf{29.5} \\
        \textbf{CS} & \cellcolor{bluebell!60}\textbf{6} & \cellcolor{bluebell!60}\textbf{8} & \cellcolor{bluebell!60}\textbf{9} & \cellcolor{bluebell!60}\textbf{11} & \cellcolor{bluebell!60}\textbf{10} & \cellcolor{bluebell!60}\textbf{12} & \textbf{1.9} & \textbf{27.4} \\
        Z & \cellcolor{gray!45}8 & \cellcolor{gray!45}10 & \cellcolor{gray!45}12 & & & & 2.0 & 31.4 \\
        SH & \cellcolor{gray!45}8 & \cellcolor{gray!45}10 & \cellcolor{gray!45}12 & & & & 2.0 & 31.4 \\
        B & 11 & & & & & & & \\
        \textbf{CW} & \cellcolor{bluebell!90}\textbf{6} & \cellcolor{bluebell!90}\textbf{7} & \cellcolor{bluebell!90}\textbf{9} & \cellcolor{bluebell!90}\textbf{10} & \cellcolor{bluebell!90}\textbf{12} & \cellcolor{bluebell!90}\textbf{13} & \textbf{1.46} & \textbf{24.1} \\
        PYM & & & & & & & & \\
        BAY & \cellcolor{gray!25}8 & \cellcolor{gray!25}11 & \cellcolor{gray!25}13 & & & & 2.5 & 32.1 \\
        LAP & \cellcolor{gray!45}8 & \cellcolor{gray!45}10 & \cellcolor{gray!45}12 & & & & 2.0 & 31.4 \\
        J & \cellcolor{gray!25}8 & \cellcolor{gray!25}11 & \cellcolor{gray!25}13 & & & & 2.5 & 32.1 \\
        SG & \cellcolor{gray!25}8 & \cellcolor{gray!25}10 & \cellcolor{gray!25}12 & & & & 2.0 & 31.4 \\
        MIN & \cellcolor{gray!45}8 & \cellcolor{gray!45}10 & \cellcolor{gray!45}12 & & & & 2.0 & 31.4 \\
        NSB & \cellcolor{gray!45}8 & \cellcolor{gray!45}10 & \cellcolor{gray!45}12 & & & & 2.0 & 31.4 \\
        ANSB & & & & & & & & \\
        \hline
    \end{tabular}
    \end{adjustbox}
    \caption{MI}
    \label{tab:Fp_tab_mi}
    \end{subtable} &
    \begin{subtable}{0.308\textwidth}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{ |l *{6}{N} : l *{2}{N} }
        \hline
        \rowstyle{} \diagbox{\emph{est}}{\emph{k}} & \rotatebox{90}{256} & \rotatebox{90}{1024} & \rotatebox{90}{4096} & \rotatebox{90}{16384} & \rotatebox{90}{65536} & \rotatebox{90}{262K} & \rotatebox{90}{Slope} & \rotatebox{90}{$l_2$-norm} \\
        \hline
        ML & \cellcolor{gray!80}4 & \cellcolor{gray!80}10 & \cellcolor{gray!80}12 & & & & 4.0 & 30.6 \\
        MM & \cellcolor{gray!45}7 & \cellcolor{gray!45}10 & \cellcolor{gray!45}12 & & & & 2.5 & 31.1 \\
        \textbf{GS\small{88}} & \cellcolor{ao(english)!55}\textbf{6} & \cellcolor{ao(english)!55}\textbf{9} & \cellcolor{ao(english)!55}\textbf{11} & \cellcolor{ao(english)!55}\textbf{13} & & & \textbf{2.3} & \textbf{29.3} \\
        GS\small{03} & \cellcolor{gray!60}7 & \cellcolor{gray!60}9 & \cellcolor{gray!60}12 & & & & 2.5 & 30.8 \\
        \textbf{SHU} & \cellcolor{ao(english)!35}\textbf{7} & \cellcolor{ao(english)!35}\textbf{9} & \cellcolor{ao(english)!35}\textbf{11} & \cellcolor{ao(english)!35}\textbf{13} & & & \textbf{2.0} & \textbf{29.5} \\
        \textbf{CS} & \cellcolor{bluebell!60}\textbf{6} & \cellcolor{bluebell!60}\textbf{7} & \cellcolor{bluebell!60}\textbf{10} & \cellcolor{bluebell!60}\textbf{12} & \cellcolor{bluebell!60}\textbf{12} & \cellcolor{bluebell!60}\textbf{12} & \textbf{2.1} & \textbf{27.9} \\
        Z & \cellcolor{gray!60}7 & \cellcolor{gray!60}9 & \cellcolor{gray!60}12 & & & & 2.5 & 30.8 \\
        SH & \cellcolor{gray!25}8 & \cellcolor{gray!25}10 & \cellcolor{gray!25}12 & & & & 2.0 & 31.4 \\
        B & 10 & & & & & & & \\
        \textbf{CW} & \cellcolor{bluebell!90}\textbf{6} & \cellcolor{bluebell!90}\textbf{7} & \cellcolor{bluebell!90}\textbf{8} & \cellcolor{bluebell!90}\textbf{13} & \cellcolor{bluebell!90}\textbf{12} & \cellcolor{bluebell!90}\textbf{13} & \textbf{1.8} & \textbf{26.2} \\
        PYM & & & & & & & & \\
        BAY & \cellcolor{gray!80}4 & \cellcolor{gray!80}10 & \cellcolor{gray!80}12 & & & & 4.0 & 30.6 \\
        LAP & \cellcolor{gray!45}7 & \cellcolor{gray!45}10 & \cellcolor{gray!45}12 & & & & 2.5 & 31.1 \\
        J & \cellcolor{gray!80}4 & \cellcolor{gray!80}10 & \cellcolor{gray!80}12 & & & & 4.0 & 30.6 \\
        SG & \cellcolor{gray!80}4 & \cellcolor{gray!80}10 & \cellcolor{gray!80}12 & & & & 4.0 & 30.6 \\
        MIN & \cellcolor{gray!25}8 & \cellcolor{gray!25}10 & \cellcolor{gray!25}12 & & & & 2.0 & 31.4 \\
        NSB & \cellcolor{gray!25}8 & \cellcolor{gray!25}10 & \cellcolor{gray!25}12 & & & & 2.0 & 31.4 \\
        ANSB & 7 & 9 & & & & & & \\
        \hline
    \end{tabular}
    \end{adjustbox}
    \caption{CMI}
    \label{tab:Fp_tab_cmi}
    \end{subtable} 
    \end{tabular}
    \label{tab:Fp_tab}
    \caption{Tabular illustration of the convergence stability for the 18 estimators of conditional mutual information $I(X;Y|Z)$. The integer values in the table represent the Flattening-off points (\emph{Fp}) of the estimations, when observed across samples of increasing size, and are calculated on the MSE. These values refer to powers of two (in line with the exponential notation used to denote sample sizes). For example, the first entry in column 2 is $4$. This indicates that the estimations obtained using the Maximum Likelihood (ML) method (for domains of size 256) exhibit negligible fluctuations ($<0.1$) when using samples bigger than $2^{4}$ (16). Equal/similar colors for the rows are used to reflect common/quasi-common flattening-off trends of the estimators over different domain sizes $k$. In bold (purple) are the faster estimators, with slight prevalence of the Chao Wang (CW) method. This observation is confirmed by the slope and Euclidean distance measurements.}
\end{table*}

==> sections/Fp_tables_orig.tex <==
\newcolumntype{N}{>{\mdseries}^w{c}{6mm}}
\begin{table}[t!]
    \large
    \begin{subtable}[t]{\columnwidth}
    \begin{adjustbox}{width=\columnwidth}
    %\begin{tabular}{ |>{\bfseries}l *{17}{^w{c}{6mm}} |}
    \begin{tabular}{ |>{\bfseries}l *{17}{N} N|}
        \hline
        \rowstyle{\bfseries} k & ML & MM & \textbf{GS\small{88}} & GS\small{03} & \textbf{SHU} & \textbf{CS} & Z & SH & B & \textbf{CW} & Pym & Bay & LaP & J & SG & Min & NSB & ANSB \\
        \hline
        256 & \cellcolor{gray!25}9 & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}\textbf{9} & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}\textbf{9} & \cellcolor{bluebell!60}\textbf{9} & \cellcolor{ao(english)!35}9 & \cellcolor{gray!25}9 & 11 & \cellcolor{bluebell!90}\textbf{9} &  & \cellcolor{gray!25}9 & \cellcolor{gray!25}9 & \cellcolor{gray!25}9 & \cellcolor{gray!25}9 & \cellcolor{gray!25}10 &  & \\

        1024 & \cellcolor{gray!25}10 & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}\textbf{9} & \cellcolor{ao(english)!35}9 & \cellcolor{ao(english)!35}\textbf{9} & \cellcolor{bluebell!60}\textbf{9} & \cellcolor{ao(english)!35}9 & \cellcolor{gray!25}10 & 13 & \cellcolor{bluebell!90}\textbf{9} &  & \cellcolor{gray!25}10 & \cellcolor{gray!25}10 & \cellcolor{gray!25}10 & \cellcolor{gray!25}10 & \cellcolor{gray!25}10 & & \\

        4096 & \cellcolor{gray!25}12 & \cellcolor{ao(english)!35}11 & \cellcolor{ao(english)!35}\textbf{11} & \cellcolor{ao(english)!35}11 & \cellcolor{ao(english)!35}\textbf{11} & \cellcolor{bluebell!60}\textbf{10} & \cellcolor{ao(english)!35}11 & \cellcolor{gray!25}12 & & \cellcolor{bluebell!90}\textbf{10} &  & \cellcolor{gray!25}12 & \cellcolor{gray!25}12 & \cellcolor{gray!25}12 & \cellcolor{gray!25}12 & \cellcolor{gray!25}12 &  & \\

        16384 & & \cellcolor{ao(english)!35}13 & \cellcolor{ao(english)!35}\textbf{13} & \cellcolor{ao(english)!35}13 & \cellcolor{ao(english)!35}\textbf{13} & \cellcolor{bluebell!60}\textbf{9} & \cellcolor{ao(english)!35}13 & & & \cellcolor{bluebell!90}\textbf{9} &  &  &  & & & & 11 & \\

        65536 & & & & & & \cellcolor{bluebell!60}\textbf{10} & & & & \cellcolor{bluebell!90}\textbf{10} & & & & & & & 12 & \\

        262K & & & & & & \cellcolor{bluebell!60}\textbf{12} & & & & \cellcolor{bluebell!90}\textbf{12} & & & & & & & & \\

        \hline
        \hline
        Slope & 1.5 & 1.33 & \textbf{1.33} & 1.33 & \textbf{1.33} & \textbf{0.5} & 1.33 & 1.5 & & \textbf{0.5} & & 1.5 & 1.5 & 1.5 & 1.5 & 1.5 & &\\

        \hline
        $l_2$-norm & 31.6 & 30.0 & \textbf{30.0} & 30.0 & \textbf{30.0} & \textbf{24.23} & 30.0 & 31.6 & & \textbf{24.23} & & 31.6 & 31.6 & 31.6 & 31.6 & 31.6 & &\\
        \hline
    \end{tabular}
    \end{adjustbox}
    \caption{H}
    \label{tab:Fp_tab_h}
    \hfill
    \end{subtable}
    
    
    \begin{subtable}[t]{\columnwidth}
    \large
    \begin{adjustbox}{width=\columnwidth}
    %\begin{tabular}{ |>{\bfseries}l *{17}{^w{c}{6mm}} |}
    \begin{tabular}{ |>{\bfseries}l *{17}{N} N|}
        \hline
        \rowstyle{\bfseries} k & ML & MM & \textbf{GS\small{88}} & GS\small{03} & \textbf{SHU} & \textbf{CS} & Z & SH & B & \textbf{CW} & Pym & Bay & LaP & J & SG & Min & NSB & ANSB \\
        \hline
        256 & \cellcolor{gray!25}8 & \cellcolor{gray!45}8 & \cellcolor{ao(english)!35}\textbf{7} & \cellcolor{gray!45}8 & \cellcolor{ao(english)!35}\textbf{7} & \cellcolor{bluebell!60}\textbf{6} & \cellcolor{gray!45}8 & \cellcolor{gray!45}8 & 11 & \cellcolor{bluebell!90}\textbf{6} & & \cellcolor{gray!25}8 & \cellcolor{gray!45}8 & \cellcolor{gray!45}8 & \cellcolor{gray!25}8 & \cellcolor{gray!25}8 & \cellcolor{gray!45}8 &\\

        1024 & \cellcolor{gray!25}11 & \cellcolor{gray!45}10 & \cellcolor{ao(english)!35}\textbf{9} & \cellcolor{gray!45}10 & \cellcolor{ao(english)!35}\textbf{9} & \cellcolor{bluebell!60}\textbf{8} & \cellcolor{gray!45}10 & \cellcolor{gray!45}10 & & \cellcolor{bluebell!90}\textbf{7} & & \cellcolor{gray!25}11 & \cellcolor{gray!45}10 & \cellcolor{gray!45}10 & \cellcolor{gray!25}11 & \cellcolor{gray!25}10 & \cellcolor{gray!45}10 &\\
        
        4096 & \cellcolor{gray!25}13 & \cellcolor{gray!45}12 & \cellcolor{ao(english)!35}\textbf{11} & \cellcolor{gray!45}12 & \cellcolor{ao(english)!35}\textbf{11} & \cellcolor{bluebell!60}\textbf{9} & \cellcolor{gray!45}12 & \cellcolor{gray!45}12 & & \cellcolor{bluebell!90}\textbf{9} & & \cellcolor{gray!25}13 & \cellcolor{gray!45}12 & \cellcolor{gray!45}12 & \cellcolor{gray!25}13 & \cellcolor{gray!25}13 & \cellcolor{gray!45}12 &\\
        
        16384 & & & \cellcolor{ao(english)!35}\textbf{13} & & \cellcolor{ao(english)!35}\textbf{13} & \cellcolor{bluebell!60}\textbf{11} & & & & \cellcolor{bluebell!90}\textbf{10} & & & & & & & & \\

        65536 & & & & & & & & & & \cellcolor{bluebell!90}\textbf{12} & & & & & & & & \\

        262K & & & & & & & & & & \cellcolor{bluebell!90}\textbf{13} & & & & & & & & \\
    
        \hline
        \hline
        Slope & 2.5 & 2.0 & \textbf{2.0} & 2.0 & \textbf{2.0} & \textbf{1.9} & 2.0 & 2.0 & & \textbf{1.46} & & 2.5 & 2.0 & 2.0 & 2.5 & 2.5 & 2.0 &\\
        \hide{
        \hline
        $l_2$-norm & 36.8 & 32.9 & \textbf{30.6} & 32.9 & \textbf{30.6} & \textbf{27.3} & 32.9 & 32.9 & & \textbf{24.0} & & 36.8 & 32.9 & 32.9 & 36.8 & 36.0 & 32.9 & \\}

        \hline
        $l_2$-norm & 32.1 & 31.4 & \textbf{29.5} & 31.4 & \textbf{29.5} & \textbf{27.4} & 31.4 & 31.4 & & \textbf{24.1} & & 32.1 & 31.4 & 31.4 & 32.1 & 32.1 & 31.4 & \\
        
        \hline
    \end{tabular}
    \end{adjustbox}
    \caption{MI}
    \label{tab:Fp_tab_mi}
    \hfill
    \end{subtable}

    \begin{subtable}[t]{\columnwidth}
    \large
    \begin{adjustbox}{width=\columnwidth}
    %\begin{tabular}{ |>{\bfseries}l *{17}{^w{c}{6mm}} |}
    \begin{tabular}{ |>{\bfseries}l *{17}{N} N|}
        \hline
        \rowstyle{\bfseries} k & ML & MM & \textbf{GS\small{88}} & GS\small{03} & \textbf{SHU} & \textbf{CS} & Z & SH & B & \textbf{CW} & Pym & Bay & LaP & J & SG & Min & NSB & ANSB \\
        \hline
        256 & \cellcolor{gray!80}4 & \cellcolor{gray!45}7 & \cellcolor{ao(english)!55}\textbf{6} & \cellcolor{gray!60}7 & \cellcolor{ao(english)!35}\textbf{7} & \cellcolor{bluebell!60}\textbf{6} & \cellcolor{gray!60}7 & \cellcolor{gray!25}8 & 10 & \cellcolor{bluebell!90}\textbf{6} & & \cellcolor{gray!80}4 & \cellcolor{gray!45}7 & \cellcolor{gray!45}7 & \cellcolor{gray!80}4 & \cellcolor{gray!80}4 & \cellcolor{gray!25}8 & 7\\

        1024 & \cellcolor{gray!80}10 & \cellcolor{gray!45}10 & \cellcolor{ao(english)!55}\textbf{9} & \cellcolor{gray!60}9 & \cellcolor{ao(english)!35}\textbf{9} & \cellcolor{bluebell!60}\textbf{7} & \cellcolor{gray!60}9 & \cellcolor{gray!25}10 & & \cellcolor{bluebell!90}\textbf{7} & & \cellcolor{gray!80}10 & \cellcolor{gray!45}10 & \cellcolor{gray!45}10 & \cellcolor{gray!80}10 & \cellcolor{gray!80}10 & \cellcolor{gray!25}10 & 9\\
        
        4096 & \cellcolor{gray!80}12 & \cellcolor{gray!45}12 & \cellcolor{ao(english)!55}\textbf{11} & \cellcolor{gray!60}12 & \cellcolor{ao(english)!35}\textbf{11} & \cellcolor{bluebell!60}\textbf{10} & \cellcolor{gray!60}12 & \cellcolor{gray!25}12 & & \cellcolor{bluebell!90}\textbf{8} & & \cellcolor{gray!80}12 & \cellcolor{gray!45}12 & \cellcolor{gray!45}12 & \cellcolor{gray!80}12 & \cellcolor{gray!80}12 & \cellcolor{gray!25}12 & \\
        
        
        16384 & & & \cellcolor{ao(english)!55}\textbf{13} & & \cellcolor{ao(english)!35}\textbf{13} & \cellcolor{bluebell!60}\textbf{12} & & & & \cellcolor{bluebell!90}\textbf{13} & 13 & & & & & & & \\
        

        65536 & & & & & & & & & & \cellcolor{bluebell!90}\textbf{12} & & & & & & & & \\
        

        262K & & & & & & & & & & & & & & & & & & \\

        \hline
        \hline
        Slope & 4.0 & 2.5 & \textbf{2.3} & 2.5  & \textbf{2.0} & \textbf{2.1} & 2.5 & 2.0 & & \textbf{1.8} & & 4.0 & 2.5 & 2.5 & 4.0 & 4.0 & 2.0 &  \\

        \hide{
        \hline
        $l_2$-norm & 39.7 & 34.7 & \textbf{31.1} & 33.7 & \textbf{31.0} & \textbf{28.0} & 33.7 & 32.9 & & \textbf{26.0} & & 39.7 & 34.5 & 34.5 & 39.7 & 39.7 & 32.9 & 30.6 \\}
        \hline
        $l_2$-norm & 30.6 & 31.1 & \textbf{29.3} & 30.8 & \textbf{29.5} & \textbf{27.9} & 30.8 & 31.4 & & \textbf{26.2} & & 30.6 & 31.1 & 31.1 & 30.6 & 30.6 & 31.4 & \\
        \hline
 
    \end{tabular}
    \end{adjustbox}
    \caption{CMI}
    \label{tab:Fp_tab_cmi}
    \end{subtable} 
    \caption{Tabular illustration of the convergence stability for the 18 estimators of entropy $H$ (a), mutual information $I(X;Y)$ (b) and conditional mutual information $I(X;Y|Z)$ (c). The integer values in the tables represent the Flattening-off points (\emph{Fp}) of the estimations, when observed across samples of increasing size, and are calculated on the MSE. These values refer to powers of two (in line with the exponential notation used to denote sample sizes). For example, the first entry in table (a) is $9$. This indicates that the estimations obtained using the Maximum Likelihood (ML) method (for domains of size 256) exhibit negligible fluctuations ($<0.1$) when using samples bigger than $2^{9}$ (512). Equal/similar colors for the columns are used to reflect common/quasi-common flattening-off trends of the estimators over different domain sizes $k$. In bold (purple) are the faster estimators, with slight prevalence of the Chao Wang (CW) method. This observation is confirmed by the slope and Euclidean distance measurements.}
    \label{tab:Fp_tab}
\end{table}
